NL-Eye: Abductive NLI for Images

Will a Visual Language Model (VLM)-based bot warn us about slipping if it detects a wet floor? Recent VLMs have demonstrated impressive capabilities, yet their ability to infer outcomes and causes remains underexplored. To address this, we introduce NL-Eye, a benchmark designed to assess VLMs' visual abductive reasoning skills. NL-Eye adapts the abductive Natural Language Inference (NLI) task to the visual domain, requiring models to evaluate the plausibility of hypothesis images based on a premise image and explain their decisions. NL-Eye consists of 350 carefully curated triplet examples (1,050 images) spanning diverse reasoning categories: physical, functional, logical, emotional, cultural, and social. The data curation process involved two steps - writing textual descriptions and generating images using text-to-image models, both requiring substantial human involvement to ensure high-quality and challenging scenes. Our experiments show that VLMs struggle significantly on NL-Eye, often performing at random baseline levels, while humans excel in both plausibility prediction and explanation quality. This demonstrates a deficiency in the abductive reasoning capabilities of modern VLMs. NL-Eye represents a crucial step toward developing VLMs capable of robust multimodal reasoning for real-world applications, including accident-prevention bots and generated video verification.

==> acknowledgements.tex <==
\section*{Acknowledgements}


==> future_work.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Currently Likely Not To Be In First VERSION SUBMISSION}
\paragraph{Visual Description Analysis.} 
\mv{MT checked - minor percentage of number hypothesis - wrong attribution and usually identifies the image - in visual baselines.}

To decouple the model's ability to correctly understand what is presented in the images from its ability to draw conclusions based on common comparative reasoning, we first set up an experiment asking the models to describe the images. We examine the models' ability to correctly identify or describe objects in the images. Distinguishing recognition from reasoning is a key step in the error analysis.


\paragraph{Contextual Challenge or Commonplace?} 
To decouple the contextual reasoning challenge from the commonplace, we assess the models' ability to retrieve the most plausible scenarios based on their general knowledge, without specific context. For example, as illustrated in the \mv{right} example in Figure \ref{fig
}, seeing a mop on the floor is generally more plausible than seeing a broom on a wet floor. However, this general plausibility may change when context is provided. In this experiment, the input consists solely of the two hypothesis images.

\mv{TODO: merge 2 pars}
To ascertain whether \bench\ truly challenges VLMs through contextualized reasoning, we test the VLM with the highest scores, \mv{model}, by experimenting with VANLI and explanation generation, but this time using only the two hypotheses and omitting the premise image. The idea is to analyze if it is possible to choose the correct hypothesis scene, even without context, to see if the model can rely on its already internal common sense.

% \subsection{Experiments}

% \paragraph{VANLI.}
% The VLI task is experimented in \mv{three} setups:
% (1) \textbf{Vanilla Setup.} The goal is to choose the plausible hypothesis given the premise. There are two frameworks: in the triplet framework (A), the task is to choose the plausible hypothesis image from two options given the premise image; in the pairs framework (B), the task is to rank the plausibility of each pair (premise and hypothesis).

% \yb{Consider splitting as well. The vanilla setup is our most relevant experiments, "vanilla" makes them sound less important. I would start with this part as the first one, and continue to additional analysis / studies, like text-only experiment to decouple X, guided task to decouple Y, etc}

\paragraph{Guiding Helps in Reasoning?}. 
The textual prompt consists of a question $\textit{Q} = \phi(\textit{Question}_M)$, while the phrasing of the question is dependent on the VLM preferable input scheme.
The goal of the following two setups is to measure the impact of accompanying the question with additional information or guidance and to explore the root of the models' difficulty.
(1) \textbf{Guided VANLI Setup.} Similar to the VANLI triplet configuration, but the question is accompanied by guidance, $\textit{P} = \phi(\textit{Question}_M, \textit{Info})$. The guidance can be temporal information, the reasoning category, hints, or all.
(2) \textbf{Chain-of-Thoughts (CoT) VLI.} Same as the Vanilla but with CoT guidance in the textual prompt, $\textit{P} = \phi(\textit{Question}_M, \textit{CoT guidance})$.\yb{What is the CoT? Currently not clear to me}

% \yb{This is a good experiment, but I think it's good to start with our main visual experiments and not the additional experiments / analysis}


\paragraph{Cross-Style Effect.} 
Human are robust to changes in visual style when it comes to reasoning \C{}.
To assess the reasoning capability dependence in consistent visual style, $\textit{S}$, in VLMs, we enrich the \bench\ with \mv{X} styles using style transfer from InstructPix2Pix \C{}. Style changes are irrelevant visual considerations in the reasoning flow of human beings \C{}. For example, showing \textit{an image of a soup} in a photorealistic style, \textit{a man holding a spoon} in an anime style, and \textit{a man holding a fork} in a vintage style won't change our logical thinking. However, we want to explore the tendencies of the models to be affected by style. The experiments include two settings: (1) \textbf{Styled VLI} and (2) \textbf{Cross-Style VLI}. The first is similar to the Vanilla setup but employs \mv{other styles} instead of just the Photorealistic style $\textit{S}_k = \rho_k(\textit{I}_i)$, and the second combines images of different styles within the same sample, $\textit{S} = \mathrm{\left\{ \rho_k(\textit{I}_p), \rho_m(\textit{I}_{h1}), \rho_n(\textit{I}_{h2}) \right\}}$, where $\textit{k,m,n}$ denote different style functions.
\yb{Do you report it in the same main table, or a seperate one? \mv{separate}}

\paragraph{Natural Images Comparison.}
\mv{Currently I think I wont do it.}

\paragraph{The "Why" make sense?:  Explanations analysis.}
\mv{cluster the explanations around consideration topics using Topic Modeling / LLM} \mv{not sure if I do it.}




Table \ref{tab:text_based reasoning} presents the performance of the textual NLI, which only receives the textual descriptions. First, we observe that the textual modality achieves the highest scores, setting the upper bound for the visual input models. The regular NLI models, DeBERTa and BART, achieve relatively high results, likely due to the greater intersection in tokens between the premise description and hypothesis 1 description.  \mv{Do this analysis!!} 

\mv{examine the cross attention maps of the failure cases?}

\paragraph{Tell the model whats true and then assess the explanation}

\paragraph{Description conditioned on task}
To me it seems like a case where the descriptions may be objectively fine, but they are not tailored to the inference task. 

For example, it might be that if you asked the model to generate the description so that it can perform the task (e.g., showing the task description and the three images in the prompt) the descriptions might have been much more suitable for the task.

==> old.tex <==



\paragraph{Baseline Configurations.}
To evaluate modern VLMs' abductive reasoning capabilities on the VANLI and Explanation Generation tasks, we define two input configurations: (1) \textit{Multiple Images} and (2) \textit{All-In-One Image}. Each configuration is tailored to a specific input format, aligning with a corresponding set of baseline models, as described in Table \ref{tab:configuration_baselines}.  The models are examined in each configuration based on their available input formats and empirical performance. For instance, Gemini-1.5 Pro Vision is a VLM capable of processing multiple images individually as well as a single image, alongside a textual prompt, making it applicable to all configurations. In contrast, LLava 1.6v, which is suited only to single-image inputs, is evaluated under configuration (2) exclusively.

 \textbf{Human Performance.} 


\paragraph{Setups.}
% To place greater emphasis on multiple-image inputs, particularly in the first two setups—\textit{Multiple Images} and \textit{All-In-One Image}—
As presented in Figure \ref{fig:setups}, for each configuration, we introduce two additional setups, the \textit{Triplet Setup} and the \textit{Pairs Setup}. Both setups require the model to predict whether a candidate hypothesis image is plausible given a premise image. However, they differ in their underlying motivation, the input format provided to the VLMs, and the expected raw output of the plausibility assessment.

% \paragraph{Pair Image Setup.} 
In the \textit{Pairs Setup}, given two images—the premise image and one candidate hypothesis image—the model assigns a numerical rank,  between 1 and 10. This process is repeated for each hypothesis-premise pair, resulting in two ranks. The hypothesis with the higher rank is considered the more plausible candidate.
The \textit{Pair} configuration is well-suited for applications like training reward models for RLHF (Reinforcement Learning from Human Feedback), generation reranking, and model selection \mv{TODO: more motivations}. 

% \paragraph{Triplet Image Setup.} 
In the \textit{Triplet Setup}, given three images—the premise and two candidate images (hypotheses)—the model identifies which candidate image is more likely (i.e., image 1 or 2, as indicated in the image or by order) and provides an explanation.
The model is correct if its choice, equals to the gold hypothesis number.
This setup is particularly useful for applications like DPO (Direct Preference Optimization) training, Theory of Mind (ToM) modeling, and mental state assessments \mv[TODO: more motivations].

% comparison - setups
% The \textit{Triplet Setup} addresses the challenge of defining a model's plausibility score in ambiguous contexts. 
In \bench, hypothesis scenarios are inherently plausible but lack a single, absolute truth for scoring. While the \textit{Pair} configuration evaluates plausibility relative to the infinite scenarios a model has encountered, the \textit{Triplet} setup simplifies this by selecting the more plausible option between two candidates, bypassing the need for meaningful ranking.

% We establish three baseline types based on their input format:
% \begin{enumerate}
%     \item[(a)] \textbf{Multimodal Models:} We use two types of multimodal models. The first type receives both text and a single image as input. The second type can handle multiple images along with text. For inputs with a single image, we use a composite image that includes all relevant images as subfigures, each with its own title. These models include \textit{Gemini Pro Vision, Claude, GPT-4-Vision, Llava 1.6, Fuyu}
%     \item[(b)] \textbf{Image-to-Text Models:} These models take images of the scenes and create detailed textual descriptions. These descriptions are then used as inputs for the language models, as described in (a). These models include \textit{Gemini Pro Vision, Claude, GPT-4-Vision, Llava 1.6, Fuyu, BLIP2-FlanT5-XL, InstructBLIP }
%     \item[(c)] \textbf{Language Models (LMs) - Textual Only:} These models, including various language models (LMs) and large language models (LLMs), receive only textual descriptions of the scenes, which may include additional information. This setup helps us measure the upper-bound reasoning abilities of the multimodal models by comparing them to text-only models. These models include \textit{Gemini Pro, Claude 3, GPT-4, Deberta v2 XL, Bart Large mnli}

% \end{enumerate}

\paragraph{Automatic Evaluation.} We evaluate the models' performance on the VANLI task using the following accuracy metrics, tailored to each setup:


%In the pair framework (i.e., premise \( I_p \) and one hypothesis \( I_{h1} \)), we ask the model to rank the plausibility \( R \) of each pair on a scale of 1-10. It is counted as correct only if the rank of the plausible hypothesis is higher than that of the implausible one, i.e., \( R(I_{h1}) > R(I_{h2}) \).

% and the difference between the ranks, ranging from 0-9, \( |R_1 - R_2|\) represents the \textit{certainty}.

(1) \textbf{Accuracy (\textit{Pairs Setup})}. When a model ranks one hypothesis as more plausible than another, the gold prediction should similarly indicate that the first hypothesis is more plausible \C{Order-Faithfulness - Nitay cite ICLR causal explanations}. It is considered correct only if the plausible hypothesis is ranked higher than the less plausible one.

\[
\text{ACC} =
\begin{cases}
1, & \text{if } (R_A > R_B \text{ when } A \text{ is plausible}) \text{ or } (R_B > R_A \text{ when } B \text{ is plausible}) \\
0, & \text{otherwise}
\end{cases}
\]

Where \(R_A\) and \(R_B\) are the ranks of pairs \(A\) and \(B\), respectively.


(2) \textbf{Accuracy (\textit{Triplet Setup})}. This measures the accuracy between the model's prediction and the gold standard selection. We identified a bias in VLMs and LLMs related to the order in which possible answers are presented \C{}. To isolate reasoning capabilities from this bias, we compute the \textit{Triplet Setup} twice: once with the plausible hypothesis presented first and once with it presented last. Accuracy is based on consistency—an answer is considered correct only if the model selects the correct option in both orders. If the model makes an incorrect selection in either order, the answer is marked as false.
A correct answer is counted only if the model is correct both times, setting the random baseline at 0.25.
\[
\text{ACC} =
\begin{cases}
1, & \text{if } C_A = C_B = \text{Gold Label} \\
0, & \text{otherwise}
\end{cases}
\]

Where \(C_A\) and \(C_B\) are the hypothesis selection of orders \(A\) and \(B\), respectively.


%The scenes tell a story that unfolds along a temporal vector, including both the temporal duration (short-term or long-term) and the direction (forward or backward) of time. This temporal vector is anchored to a specific scene, known as the context scene, which serves as the reference point from which the rest of the story is presented. } 



% (2) \textbf{Certainty}. In the triplet framework, certainty is the probability \( p \) provided by the models. In the pair framework, it is computed as the difference between the ranks, ranging from 0 to 9, i.e., \( p = R(I_{h1}) - R(I_{h2}) \).

% \paragraph{Plausibility Prediction.} 
% The results of the VLM's with input of single image (all in one image) are presented in Table \ref{tab:evaluation} \mv{on all 350} and Figure \ref{fig:category_all_in_one} \mv{currently of only 93 samples}. 


% tables results - separate
% \begin{table}[ht]
% \centering
% % \begin{minipage}{0.45\textwidth}
% % \small
% % \setlength{\tabcolsep}{1pt} % Reduce column padding
% \begin{adjustbox}{width=0.65\textwidth}
% \begin{NiceTabular}{ll|cc|cc}
% \toprule
% &  & \multicolumn{2}{c}{\textbf{Prediction}} & \multicolumn{2}{c}{\textbf{Explanation}} \\
% % \cline{3-6}
%  % & &  \multirowcell{2}{\textbf{Acc} \\ Triplet} & \multirowcell{2}{\textbf{Acc} \\ Pairs} & \multirowcell{2}{\textbf{Human} \\ Eval} & \multirowcell{2}{\textbf{Auto} \\ Eval} \\
%  \textbf{Strategy} & \textbf{Model} & Triplet & Pairs & Human & Auto \\
% \midrule
% \multirowcell{4}{\textbf{Multiple} \\ \textbf{Images}} 
%  & Gemini-Pro-Vision 1.5 &  \textbf{51}\% & 42\% & 38\% & 34\%\\
%  & GPT-4-Vision &  46\% & 40\% & 36\% & 37\%\\
%  & GPT-4o &  16\% & \textbf{50}\% & 23\% & 23\%\\
%  & Claude-Sonnet-3.5 &  \textbf{49}\% & \f{38}\% & 51\% & 26\%\\
% \midrule
% \multirowcell{6}{\textbf{All-in-One} \\  \textbf{Image}} 
%  & Gemini-Pro-Vision 1.5 &  43\% & 39\% & 41\% & 33\%\\
%  & GPT-4-Vision &  41\% & 34\% & 41\% & 27\%\\
%  & GPT-4o &  \textbf{60}\% & \textbf{45}\% & 37\% & 40\%\\
%  & Claude-Sonnet-3.5 &  28\% & \mv{} & 26\% & 21\%\\
%  & Claude-Opus-3 & 15\% & \mv{} & 25\% & 6\%\\
%  & LLaVA 1.6 &  14\% & 42\% & 14\%  & 4\%\\
%  & Fuyu &  4\% & 44\% & 10\% & 2\%\\
% \midrule
% & \textbf{Random} &  25\% &  45\% &  & \\
% & \textbf{Dumb Pixel} & 50\% &  50\%&  & \\
% \hline
% & \textbf{Humans} & \textbf{85}\% &  \f{83}\%&  \textbf{94}\%& \\
% \bottomrule
% \end{NiceTabular}
% \end{adjustbox}
% \caption{Performance of Visual-based Reasoning baselines on the VANLI and explanation generation.}
% \label{tab:visual_based_rasoning}
% \end{table}
% % \end{minipage}%

% % \hfill
% % \begin{minipage}{0.45\textwidth}

% \begin{table}[ht]
% \centering
% \footnotesize
% \begin{adjustbox}{width=0.65\textwidth}
% \begin{NiceTabular}{l l|l|c}
% \toprule
% \multirowcell{2}{\textbf{Strategy}} & \multirowcell{2}{\textbf{Describer}} & \multirowcell{2}{\textbf{Predictor}} & \multirowcell{2}{\textbf{Accuracy} \\ \textit{Triplet}} \\
% & & & \\
% \midrule
% \multirow{7}{*}{\textbf{Text-Only}} 
%  & \multirow{6}{*}{Gold} 
%  & Gemini-Pro 1.5 & 66\% \\
%  & & GPT-4o & \textbf{80}\% \\
%  & & GPT-4 & \textbf{78}\% \\
%  & & Claude-Sonnet-3.5 & \textbf{79}\% \\
%  & & Claude-Opus-3 & \textbf{81}\% \\
%  & & BART L mnli & 68\% \\
%  & & \f{DeBERTa nli v3} & 65\% \\
%  & & DeBERTa XL v2 & 50\% \\
% \midrule
% \multirow{7}{*}{\textbf{Image-to-Text}} 
%  & Gemini pro vision & GPT-4o & 29\% \\
%  & GPT-4 vision &  & 32\% \\
%  & Claude 3.5\textsuperscript{*} &  & \textbf{39}\% \\
%  & Claude 3\textsuperscript{*} &  & 33\% \\
%  & LLaVA 1.6 &  & 29\% \\
%  & BLIP 2 &  & \textbf{40}\% \\
%  & Instruct BLIP &  & 35\% \\
% \bottomrule
% \end{NiceTabular}
% \end{adjustbox}
% \caption{Performance of Textual-based Reasoning approach on the VANLI and explanation generation. The predictors, i.e. reasoners, rely on the gold textual descriptions, and the Image-to-Text model descriptions. * indicates reliance on a subset of the data \footnote{Descriptions of 193 examples due to Anthropic API constraints.}}
% \label{tab:text_based_reasoning}
% % \end{minipage}
% \end{table}



% The abductive reasoning capabilities of VLMs are derivatives of more fundamental visual skills. While the entire model contributes to reasoning abilities, for simplicity, we can examine the model’s components separately since each serves distinct functions: the visual encoder, responsible for visual interpretations, and the language model (LM), responsible for reasoning.

% In the text-only approach, the input consists solely of concise, gold-standard textual descriptions, which contain all the information necessary for correct reasoning. In the image-to-text approach, we assess the VLM's ability to interpret images accurately enough to provide sufficient information for reasoning success.


% analysis:
% \mv{Recall, Precision, F1, Cohen's Kappa - Triplet + Pairs, per model, average across models from the same baseline type}

% Examining the failures of human choices and VLMs (Multiple Images, Triplet Setup), across all 350 examples (see full comparison in Appendix Table \ref{app_tab:human_models_correct}), we observe several trends. When humans are correct, the model succeeds 66\% of the time, suggesting that what is easier for humans is also more likely to be easier for models. However, when humans are incorrect, the model's success rate drops to a random chance of 50\%. Overall, the average agreement between humans and models is 64\%.

% The percentage of instances where the model is correct but the human is not is minimal (7\%). In such cases, it is rare for the model's explanation to be correct. Figure \mv{TODO: Fig} illustrates a rare example of this scenario. 
% When the model fails, only about 22\% of these failures are shared with humans, meaning both the model and the human answer incorrectly. This indicates that different types of errors are present in the common reasoning patterns of humans and models.

% dataset creation:
% \yb{A point that may come up: why can't this process be automated? The answer (that I know) is that human involvement is needed to make sure the scene is aligned with the text, and that there are consistency in the details between scenes. If this is correct, consider diving into this difficulty: at least explaining it here \mv{added in the beginning.}, and even adding a figure showing this complexity. This point came up in WHOOPS! rebuttal, and we added Figure 4 to address it \mv{\ref{fig:images_gen_zoom_in}}\url{https://arxiv.org/pdf/2303.07274}.}
% \zg{I think that you should discuss the human eval here as another subsection. I know that this is also a baseline, but (more importantly) this is also a tool that validates the validity of your dataset.}

% ------- intro ---- old:

% \green{Modern VLMs have already been tested across a variety of challenging tasks including visual entailment and detecting improbable events (e.g., fire in a closed jar).
% However, exisiting evaluation typically considered sequential scenes (such as next-frame prediction), or in a single scene setting (such as visual entailment or detecting improbable events like a fire in a closed jar) \cite{xie2019visual,   Fu2022TheresAT, hessel2022abduction,fu2024blink,ganz2024question,yarom2024you}. 
% This make it not clear whether exiting VLMs are capable of abductive reasoning.}

% % common sense
% % , drawing significantly on visual understanding, general knowledge, and reasoning abilities
% Common sense plays a pivotal role in human cognition and interaction with the world \cite{smith1995formal} \C{ more 2-3 cognition updated work}. \textit{Abductive reasoning}, is the ability to infer and predict plausible outcomes or causes given a context scene \cite{peirce1934pragmatism, fann2012peirce, sep-abduction}. \zg{I strongly suggest to think on intuitive example of abductive reasoning and give it here. You can then use it as a running example to explain concepts.} \f{Justifying hypotheses—whether observed or as mental states—by assessing their relative plausibility and providing an explanation} is suggested as a distinctive feature of human cognition compared to lower species. \cite{magnani2009abductive}. 

% % Models and common sense
% \zg{You can easily just start with this, and integrate a bit of stuff from the previous paragraph here.}
% As multimodal AI, specifically Visual Language Models (VLMs) become more integrated into our daily lives \C{ even links to apps/companies}, their ability to monitor and interpret scenes will be crucial. They will need to correctly infer plausibility to prevent accidents and provide timely advice. Questions one may ask are, for example, whether a bot would warn us about leaving the gas on next to a towel, or would it notify us if a crying baby simply dropped a pacifier? \zg{Great, now is the place to explain how these cases are manifested in abductive reasoning.}
% \f{The answer depends on the bot's abductive reasoning, requiring an assessment of the plausibility of fire as an outcome compared to a false warning, or the missing pacifier relative to other possible causes, along with the ability to justify these conclusions through explanation.}

% % This in turn requires higher cognitive perception in AI models, leveraging visual input signals with the ability to communicate with us \zg{This sentence is vague and not helping the motivation.}

% % \yb{Perhaps it will be interesting to add somewhere a motivation also for video generation, where we can control the plausibility of the next scene} 

% % problem - related work
% However, VLMs have primarily been tested on isolated features in simple, sequential scenes, such as next-frame prediction, or in a single scene, such as visual entailment or detecting improbable events (e.g., fire in a closed jar) \cite{xie2019visual,   Fu2022TheresAT, hessel2022abduction,fu2024blink,ganz2024question,yarom2024you}. These models have not been \f{thoroughly} assessed \f{yet} in complex common-sense scenarios that involve temporal leaps and require a deep understanding of the world and human dynamics based on multiple visual inputs \zg{The last sentence should be clearly motivating abductive reasoning, right not it is not}.


% solution - the main contribution
% To address gaps in the current literature and facilitate deeper analysis of VLMs' reasoning capabilities, \zg{Start thrsentence from here}
% \f{In this work, we introduce the \bench, a \textit{novel} benchmark designed to evaluate \textit{multi-image visual abductive reasoning capabilities} of VLMs. In NLP, the reasoning capabilities of language models are often tested using the abductive NLI \cite{bhagavatula2019abductive} task, which assesses whether a sentence can be inferred from another \zg{This sounds like your motivation is simply since there is a task like this in NLP, but as you mention before, your motivation is much more than that.}. Similarly, our approach adapts this evaluation to the visual domain, offering a distinct perspective compared to other benchmarks.}

% benchmark tasks
% The \task\ task evaluates a model's reasoning capabilities by assessing the plausibility of a hypothesis image based on a given context image. \zg{I think that for the average reader it will not be clear now what is abductive NLI, and it should be in order to understand the next sentence. The reader understands that it has something to do with "assessing the plausibility of a hypothesis" but it should be more specific at this point.}
% Our benchmark consists of two main tasks: Visual Abductive Natural Language Inference (\task) and Explanation Generation. In the \task\ task, a VLM is given a premise image and one or two hypothesis images. It needs to infer how likely (plausible) each hypothesis image is to lead to or result from the context image, both individually and in comparison to the other hypothesis. The premise scene is crucial for determining the more plausible hypothesis. Without it, accurately judging which scene is more plausible becomes nearly impossible. \zg{The explanation of the main task still needs improvement, it should be more TAHLES.} 
% We also evaluate the models' ability to provide faithful explanations for their decisions, to explore whether they are correct from the right reasons rather than shallow heuristics \cite{mccoy-etal-2019-right}. For example, a valid explanation for the broken leg scene would suggest that the presence of a warning sign would have made the man more alert, thereby potentially preventing the accident. In contrast, a shallow explanation might suggest that the man was simply resting on a cozy rainy day.


%Our work focuses on inferring the most plausible hypothesis image by addressing missing, ambiguous, or implied information as the explanation.

% The \bench\ sample consists of a triplet of images, contains one premise \footnote{We use interchangeably the terms premise image and context image \zg{Why not pick a terminology and be consistent?}.} and two hypotheses\footnote{We use interchangeably the terms the hypothesis image or candidate image \zg{Why not pick a terminology and be consistent?}.}, where one is more plausible than the other given the premise image.
%The VLM receives the images and is prompted to determine which hypothesis image is more plausible (triplet setup) or rank how plausible (pair setup) given the premise image.}  
% The scene triplet structure of the samples supports two configurations for examining these tasks: the pair configuration and the triplet configuration. In the pair setup, one candidate scene is evaluated given the context, whereas in the triplet setup, one candidate scene is evaluated in relation to another candidate and the premise. The pair setup is more suited for retrospective examination (such as in video generation verification), while the triplet setup is better for planning (simulating multiple options) or training reward policies.

% \nc{maybe present as 4 tasks: The scene triplet in our benchmark supports four novel visual reasoning tasks, two involving predicting whether a candidate image is plausible given a context image: (1) selecting the more plausible scene between the two; (2) scoring the plausibility of a candidate image.
% The other two tasks involve explaining why a candidate scene can occur, given the context: (3) generating a contrastive explanation in the form of "why A instead of B" - "why candidate A is more plausible to occur than candidate B given the context image?"; (4) answering "why A" - "why candidate A can occur?"
% }

% \yb{In this part, or in the previous one, it's good to refer to Figure \ref{fig:main_nl-eye}, and explain the tasks using it \zg{$+1$}}
% \yb{I propose to mention both the triplet and pairs image-image NLI tasks. Emphasizing that AFAIU NLI is more expected to run on pairs rather than a triplet so this is why I think adding the pairs will be helpful}
 % \zg{The terminology is confusing, in the previous paragraph you described the benchmark and now you do it again, what is the logical devision between paragraphs? Maybe you first describe the dataset and then the Benchmark?}
 % \zg{"consensus human explanation" is not clear, why human explanation? The task is performed by a model. Separate the dataset from the task in your terminology.}
% \yb{consider rephrasing to something like "we also evaluate the models ability to provide faithful explanations for their decisions, and making sure they are correct from the right reasons rather than shallow heuristic (+relevant paper: https://aclanthology.org/P19-1334/)"}.

 
% \bench\ consists 350 examples, each containing a premise image and two hypothesis images, as well as a gold-label indicating the index of the more plausible hypothesis. To generate the images, we first collect a large pool of high-quality textual scenes which are created with \emph{human-annotators}. To ensure high quality of the scenes, this part is done by experienced NLP researchers. The scenes then undergo extensive filtering by additonal human annotators according to multiple criterias (e.g. "the premise must be essential for determining the more plausible hypothesis"). After that we are left with 350 scenarios which are then given to designers who employ Midjourney and DALL-E\yb{citations?} to synthesize the images.

% The images were generated based on textual scenes that were carefully collected from human annotators. 

% (i.e. a total of 1050 images).  human-handcrafted scenes, depicted by their textual description,  generated images, and gold explanations for plausibility. It is divided into 350 samples carefully designed and filtered. Designers employ Midjourney and DALL-E\yb{citations?} to synthesize the images' scenes, ensuring high-quality visual consistency within the same sample scenes. In \S \ref{sec:collection} we present the benchmark building process.

% \bench\ consists of 1050 human-handcrafted scenes, depicted by their textual description,  generated images, and gold explanations for plausibility. It is divided into 350 samples carefully designed and filtered. Designers employ Midjourney and DALL-E\yb{citations?} to synthesize the images' scenes, ensuring high-quality visual consistency within the same sample scenes. In \S \ref{sec:collection} we present the benchmark building process.

% \zg{What designers? You did not mention any designers.}


% Moreover, the \bench\ benchmark enables evaluating multiple reasoning capabilities and analyzing when VLMs fail. The benchmark covers a diverse array of relationships between the premise scene and the hypothesis scenes, requiring the VLM to hold different types of reasoning capabilities. This includes the temporal reasoning direction: forward, backward, or simultaneously, as well as the temporal term: short-term and long-term. In addition, the benchmark covers six reasoning categories: physical, logical, emotional, functional, cultural, and social (see Figure \ref{fig:main_nl-eye}).
% The broad diversity of the \bench\ benchmark aids in diagnosing current VLMs and highlights their weaknesses.

% abstract - drafts:

% \mt{I’d avoid using the term "abductive reasoning" before providing an explanation.
% avoid using parentheses. Also, add a more substantial statement about the results. Something like: "Gemini and GPT achieved the best performance, underperforming humans by X. The explanations are generally accurate when the correct answer is selected, and there is a logical sense when it is wrong. However, a significant gap remains, mainly due to missing key details, and..."
% }
% draft 1:
% Recent years have seen significant advances in visual-language capabilities; however, these have primarily been assessed through foundational tasks such as object detection, which do not account for reasoning between multiple scenes. This paper introduces the \bench\, a benchmark designed to evaluate the visual abductive reasoning capabilities across Visual Language Models (VLMs). Adapting the Natural Language Inference (NLI) task to the visual domain involves reasoning about the plausibility of two visual scenarios (hypotheses) based on a premise image and providing an explanation for the rationale behind the decision. \bench\ consists of 350 examples, each depicted through textual descriptions and synthesized images. The \bench\ benchmark tests VLMs across different input strategies and setups. We analyze the performance and find a significant gap compared to humans. In some cases, the performance even lags behind random or degraded baselines. This evaluation is vital as a fundamental step toward enhancing multimodal reasoning and the cognitive capabilities of VLMs in human-AI collaborative environments—such as accident prevention AI tools, autonomous vehicles, and AI-generated video verification.\footnote{Our code and data will be made available.} 

%This evaluation is crucial for advancing conditional video generation, emphasizing the importance of multimodal reasoning and temporal commonsense. \footnote{Our code and data will be made available.}

% \zg{This also sais nothing. Why it is vital? Should the reader just trust you on this? Avoid claims that you do not support, especially in the abstract where the space is really expensive.}
% \zg{(1) You do not just introduce a benchmark, but also a new task. (2) Per my previous comment: there is no motivation for Abductive Reasoning and the only motivation you give is lack of temporal dimension which is not related.}

% In recent years, Visual Language Models (VLMs) have demonstrated impressive capabilities, yet their ability to perform reasoning across multiple images remains underexplored.
% To address this gap, we introduce \bench, a novel benchmark designed to evaluate the visual abductive reasoning capabilities of VLMs. \bench\ adapts the Natural Language Inference (NLI) task from text to the visual domain, requiring models to assess the plausibility of hypothesis images based on a given premise image and explain their decisions. The benchmark features 350 carefully curated examples, each depicted through textual descriptions and synthesized images, and challenges VLMs to reason in diverse scenarios, including physical, logical, emotional, cultural, and social categories.
% Our experiments show that current leading VLMs struggle significantly with visual abductive reasoning, while human performance excels in predicting plausibility and providing quality explanations. Moreover, the performance of most VLMs is similar to random baselines.
% Through extensive analysis, we found that VLMs exhibit inconsistency and struggle with visual interpretation and knowledge integration across multiple images. We believe the \bench\ benchmark represents a significant step toward developing VLMs capable of robust multimodal reasoning for real-world applications, such as safety-critical AI systems, autonomous agents, and synthetic video verification.
%  \footnote{Our data and code will be available upon acceptance.}

% draft 2:
% In recent years, Visual-Language Models (VLMs) have demonstrated impressive capabilities in foundational tasks, yet their ability to perform reasoning across complex scenarios remains underexplored. To address this gap, we introduce \bench, a novel benchmark designed to evaluate the visual abductive reasoning abilities of VLMs across multiple images. \bench adapts the Natural Language Inference (NLI) task from text to the visual domain, requiring models to assess the plausibility of hypotheses based on a given premise image and generate explanations for their decisions. Featuring 350 carefully curated examples, each depicted through textual descriptions and synthesized images, the benchmark challenges VLMs to reason across diverse scenarios, including physical, logical, emotional, cultural, and social categories. Our experiments reveal that current leading VLMs struggle significantly with these tasks, with most models failing to outperform random baselines, while human performance excels in both predicting plausibility and providing high quality explanations. A key finding suggests that while VLMs possess some reasoning capabilities, these are hindered by weak visual interpretation.  \bench provides a crucial step toward developing VLMs capable of robust multimodal reasoning for real-world applications, such as safety-critical AI systems and autonomous agents, or synthetic video verification. \footnote{All data and code will be made available.}

% \nc{maybe present as 4 tasks: The scene triplet in our benchmark supports four novel visual reasoning tasks, two involving predicting whether a candidate image is plausible given a context image: (1) selecting the more plausible scene between the two; (2) scoring the plausibility of a candidate image.
% The other two tasks involve explaining why a candidate scene can occur, given the context: (3) generating a contrastive explanation in the form of "why A instead of B" - "why candidate A is more plausible to occur than candidate B given the context image?"; (4) answering "why A" - "why candidate A can occur?"
% }

% \yb{I propose to indicate the two tasks (or subtasks) of triplet or pairs image-image NLI. By the way, the pairs NLI can be also run with the textual models.}


%%%% OLDDDDDDDDDDDD


% \section{OLD - remove}



% As output it generates a choice (one of the hypothesis number), $\textit{C}$, and an explanation, $\textit{E}$. 



% \mv{TODO:? where explanations}
% \paragraph{Explanations.} Models and human beings provide various explanations, which we rate for their fitting to the samples and then sort. Creating a set of acceptable explanations is an integral part of the \bench\ benchmark. Moreover, we cluster the explanations around consideration topics using \mv{Topic Modeling / LLM}. The goal of mapping the explanations into groups is to enhance our understanding of the different models' focus areas and sensitive zones.\yb{Do we have explanations only to the triplet or the pairs too?}


% \textbf{Explanations Evaluation By Humans.} Evaluating explanations is a challenging task due to its open-ended nature: there can be multiple acceptable answers, variations in phrasing, and the need for high logical reasoning skills \C{}. After collecting the explanations generated by the models, \( E_m \), and the human annotators, resulting in \mv{Y} explanations, we create a second task on MTurk to evaluate the validity of the explanations and their quality. \mv{Z} crowd-workers select the explanations that are correct for each specific sample.

% The task involves multiple-choice questions where there may be more than one valid explanation. The explanations are taken from all the experimented models and human annotators, but only from cases where they correctly chose the plausible hypothesis in the VANLI task. See more details in Appendix \S \mv{S}.

% We compute the mean accuracy for each model, \( R_m \), which represents how often the model's explanation was chosen as correct among all cases. The mean rank is given by:

% \[
% Human Rating = \frac{N_{E_m}}{N_m}
% \]

% where \( N_{E_m} \) is the number of explanations generated by model \( m \) that were chosen as valid, and \( N_m \) is the total number of explanations generated by model \( m \) in the evaluation set.

% breakdowns categoires:




% \mv{TODO: Reasoning Categories Breakdown}
% Second, There is a variation in the performance across different reasoning categories. The \mv{Social and Logical} categories found to be the most intuitive, scoring with \mv{X and Y} accuracy. 

% \begin{table}[!h]
%     \centering
%     \small
%     \setlength{\tabcolsep}{1pt} % Reduce column padding
%     \begin{tabular}{|l|c|c|c|c|c|}
%         \hline
%         \textbf{Model} & \textbf{Category} & \textbf{Plausible - Accuracy} & \textbf{Plausible - F1} & 
%         \textbf{Exp. (HR)} & 
%         \textbf{Exp. (Auto)} \\
%         \hline
%         \multirow{1}{*}{Gemini-Pro-Vision} 
%         % & Physical & & & & \\
%         % \cline{2-6}
%         % & Social & & & & \\
%         % \cline{2-6}
%         % & Emotional & & & & \\
%         % \cline{2-6}
%         % & Functional & & & & \\
%         % \cline{2-6}
%         % & Cultural & & & & \\
%         % \cline{2-6}
%         % & Logical & & & & \\
%         % \cline{2-6}
%         & Overall & & & & \\
%         \hline
%         \multirow{1}{*}{Claude-Opus-3}
%         % & Physical & & & & \\
%         % \cline{2-6}
%         % & Social & & & & \\
%         % \cline{2-6}
%         % & Emotional & & & & \\
%         % \cline{2-6}
%         % & Functional & & & & \\
%         % \cline{2-6}
%         % & Cultural & & & & \\
%         % \cline{2-6}
%         % & Logical & & & & \\
%         % \cline{2-6}
%         & Overall & 0.302 (order: hyp1) & & & \\
%         \hline
%         \multirow{1}{*}{Claude-3.5}
%         % & Physical & & & & \\
%         % \cline{2-6}
%         % & Social & & & & \\
%         % \cline{2-6}
%         % & Emotional & & & & \\
%         % \cline{2-6}
%         % & Functional & & & & \\
%         % \cline{2-6}
%         % & Cultural & & & & \\
%         % \cline{2-6}
%         % & Logical & & & & \\
%         % \cline{2-6}
%         & Overall & & & & \\
%         \hline
%         \multirow{1}{*}{GPT-4-Vision}
%         % & Physical & & & & \\
%         % \cline{2-6}
%         % & Social & & & & \\
%         % \cline{2-6}
%         % & Emotional & & & & \\
%         % \cline{2-6}
%         % & Functional & & & & \\
%         % \cline{2-6}
%         % & Cultural & & & & \\
%         % \cline{2-6}
%         % & Logical & & & & \\
%         % \cline{2-6}
%         & Overall & 0.411 (both) |0.545 (ord: hyp1) | 0.671 (hyp2) & & & \\
%         \hline
%         \multirow{1}{*}{Gemini-Pro-Vision}
%         % & Physical & & & & \\
%         % \cline{2-6}
%         % & Social & & & & \\
%         % \cline{2-6}
%         % & Emotional & & & & \\
%         % \cline{2-6}
%         % & Functional & & & & \\
%         % \cline{2-6}
%         % & Cultural & & & & \\
%         % \cline{2-6}
%         % & Logical & & & & \\
%         % \cline{2-6}
%         & Overall & 0.424 (both) | 0.454 (ord: hyp1, 339 samples) | 0.824 (ord hyp2) & & & \\
%         \hline
%         \multirow{1}{*}{Llava 1.6v}
%         % & Physical & & & & \\
%         % \cline{2-6}
%         % & Social & & & & \\
%         % \cline{2-6}
%         % & Emotional & & & & \\
%         % \cline{2-6}
%         % & Functional & & & & \\
%         % \cline{2-6}
%         % & Cultural & & & & \\
%         % \cline{2-6}
%         % & Logical & & & & \\
%         % \cline{2-6}
%         & Overall & 0.14 (both correct) | 0.53 (ord hyp1) | 0.26 (ord hyp2)& & & \\
%         \hline
%         \multirow{1}{*}{Fuyu-8b}
%         % & Physical & & & & \\
%         % \cline{2-6}
%         % & Social & & & & \\
%         % \cline{2-6}
%         % & Emotional & & & & \\
%         % \cline{2-6}
%         % & Functional & & & & \\
%         % \cline{2-6}
%         % & Cultural & & & & \\
%         % \cline{2-6}
%         % & Logical & & & & \\
%         % \cline{2-6}
%         & Overall & & & & \\
%         \hline
%     \end{tabular}
%     \caption{Evaluation of Models Across Different Categories. Exp. stands for Explanations, HR for Human Rate.}
%     \label{tab:evaluation}
% \end{table}

% \begin{table}[!h]
%     \centering
%     \small
%     \setlength{\tabcolsep}{1pt} % Reduce column padding
%     \begin{tabular}{|l|c|c|c|c|c|}
%         \hline
%         \textbf{Model} & \textbf{Category} & \textbf{Plausible - Accuracy} & \textbf{Plausible - F1} & 
%         \textbf{Exp. (HR)} & 
%         \textbf{Exp. (Auto)} \\
%         \hline
%         \multirow{1}{*}{GPT 4} 
%         % & Physical & & & & \\
%         % \cline{2-6}
%         % & Social & & & & \\
%         % \cline{2-6}
%         % & Emotional & & & & \\
%         % \cline{2-6}
%         % & Functional & & & & \\
%         % \cline{2-6}
%         % & Cultural & & & & \\
%         % \cline{2-6}
%         % & Logical & & & & \\
%         % \cline{2-6}
%         & Overall & 0.78 (both) |0.868 (ord: hyp1) | 0.82 (hyp2) & & & \\
%         \hline
%         \multirow{1}{*}{Claude Opus 3} 
%         % & Physical & & & & \\
%         % \cline{2-6}
%         % & Social & & & & \\
%         % \cline{2-6}
%         % & Emotional & & & & \\
%         % \cline{2-6}
%         % & Functional & & & & \\
%         % \cline{2-6}
%         % & Cultural & & & & \\
%         % \cline{2-6}
%         % & Logical & & & & \\
%         % \cline{2-6}
%         & Overall & 0.805 (both) | 0.854 (order: hyp1)| 0.874 (hyp2) & & & \\
%         \hline
%         \multirow{1}{*}{Gemini Pro} 
%         % & Physical & & & & \\
%         % \cline{2-6}
%         % & Social & & & & \\
%         % \cline{2-6}
%         % & Emotional & & & & \\
%         % \cline{2-6}
%         % & Functional & & & & \\
%         % \cline{2-6}
%         % & Cultural & & & & \\
%         % \cline{2-6}
%         % & Logical & & & & \\
%         % \cline{2-6}
%         & Overall & 0.658 (both)| 0.725 (ord: hyp1)| 0.79 (hyp2) & & & \\
%         \hline
%         \multirow{1}{*}{bart large mnli} 
%         % & Physical & & & & \\
%         % \cline{2-6}
%         % & Social & & & & \\
%         % \cline{2-6}
%         % & Emotional & & & & \\
%         % \cline{2-6}
%         % & Functional & & & & \\
%         % \cline{2-6}
%         % & Cultural & & & & \\
%         % \cline{2-6}
%         % & Logical & & & & \\
%         % \cline{2-6}
%         & Overall & 0.68 & & & \\
%         \hline
%         \multirow{1}{*}{deberta v2 xlarge} 
%         % & Physical & & & & \\
%         % \cline{2-6}
%         % & Social & & & & \\
%         % \cline{2-6}
%         % & Emotional & & & & \\
%         % \cline{2-6}
%         % & Functional & & & & \\
%         % \cline{2-6}
%         % & Cultural & & & & \\
%         % \cline{2-6}
%         % & Logical & & & & \\
%         % \cline{2-6}
%         & Overall & 0.49 & & & \\
%         \hline
%     \end{tabular}
%     \caption{Textual NLI: Evaluation of Models Across Different Categories. Exp. stands for Explanations, HR for Human Rate.}
%     \label{tab:evaluation_textual}
% \end{table}



% \f{Multi-image abductive reasoning requires skills beyond single-image tasks. While single-image reasoning involves basic object detection and recognition, multi-image reasoning demands more advanced abilities like integrating information across images, tracking objects, and understanding changes in perspective. As tasks grow more complex, further capabilities are needed, such as retrieving global knowledge, connecting the dots, considering social and cultural sensitivities, and assessing the plausibility of sequences with clear logical explanations.} \zg{This seems like a continuation of the motivation part in the intro section. This is not the place for that, here you need to explain what this section is about.}

% Based on the \bench\ tasks and input strategies, we suggest further analyses setups which aim to isloate different aspects in the inference process of the models and test their effect on the final task performance:


% The motivation for using various configurations arises from the need to evaluate a wide range of VLMs and 

% To assess VLMs reasoning capabilities by isolating the contributions of each component—namely, the textual decoder (LM) and the visual encoder—to the overall performance, we examine two additional configurations: \textit{Text-Only} and \textit{Image-to-Text}.

% \begin{itemize}
%     \item \textbf{Inaccurate assumptions about reality} (e.g., misinterpreting a distressed firefighter or a human gesture in a gambling scene).
%     \item \textbf{Failure to account for time duration and age differences} (e.g., misunderstanding the time duration in the context of a child's vaccination).
%     \item \textbf{Missing visual knowledge} (e.g., unfamiliarity with crossed fingers in a gambling game).
%     \item \textbf{Over-sensitivity hindering reasoning} (e.g., overly accepting interpretations that hinder reasoning, such as assuming a crying firefighter during a fire is acceptable).
%     \item \textbf{Overlooking key details} (e.g., missing a man’s facial expression of happiness in a hospital, despite recognizing him).
%     \item \textbf{Style-based reasoning} rather than focusing on substance.
%     \item \textbf{Lack of multi-hop reasoning} needed to connect multiple pieces of information.
% \end{itemize}

\paragraph{Input Strategies} Traditionally, visual tasks have involved reasoning about a single image, so most vision models and visual-language models (VLMs) were developed to process one image at a time. However, with the recent shift towards chat-based VLMs, many models now have the capability to process multiple images. We experiment with two strategies for feeding visual input to the model: (1) \textit{\combined} -- where we concatenate the images (with the premise on the left) to form a single combined image, and (2) \textit{\separate}  -- where we feed the images to the model one at a time\yb{one at a time sounds like it's a dialog, while we mean to models that are able to process several images. Consider rephrasing to make it clearer}, starting with the premise. As not all models support both strategies, Table~\ref{tab:model-usage} specifies which strategy was used for each model in our study. 

\paragraph{Reasoning Approaches} To thoroughly assess the abductive reasoning capabilities of current models, we use two reasoning approaches: (1) \textit{Visual-based} -- where the model is tasked with performing the entire task end-to-end based solely on the visual input, and (2) \textit{Textual-based} -- where the final plausibility reasoning is based on textual input. In this approach, we first ask the model to describe the two images in natural language, and then, using those descriptions, the same model or another performs the plausibility prediction. We refer to this procedure as \textit{image-to-text}. Alternatively, in the \textit{text-only} procedure, we can discard the visual inputs altogether and use only the textual descriptions generated when the images were created (see \S\ref{sec:creation}).
The visual-based and textual-based approaches allow us to understand the model's weaker capabilities better.

\paragraph{Reasoning Approaches \& Input Strategies} To thoroughly assess the abductive reasoning capabilities of current models, we use two reasoning approaches: (1) \textit{Visual-based} -- where the model is tasked with performing the entire task end-to-end based solely on the visual input, and (2) \textit{Textual-based} -- where the final plausibility reasoning is based on textual input.

\f{In the visual-based approach, we experiment with two \textbf{Input Strategies} for feeding input to the model: (1) \textit{\combined} -- where we concatenate the images (with the premise on the left) to form a single combined image, and (2) \textit{\separate}  -- where we feed the images to the model separately in one prompt}, starting with the premise. As not all models support both strategies, Table~\ref{tab:model-usage} specifies which strategy was used for each model in our study. 

In the textual-based approach, we utilize two input strategies as well: (1) \textit{image-to-text} -- where we ask the model to describe the two images in natural language, and then, using those descriptions, the same model or another performs the plausibility prediction, and (2) \textit{text-only} -- we discard the visual inputs altogether and use only the textual descriptions generated when the images were created (see \S\ref{sec:creation}).

The visual-based and textual-based approaches allow us to understand the model's weaker capabilities better.


% \mv{--Just thoughts right now--}
% %discussion benchmark
% The task characteristics reveal unique and challenging elements in the benchmark annotations \zg{How a characteristics of a task can reveal anything? Maybe your study can...}. Though transferring to the visual domain demonstrates better the human experience, it also leads to more open and subjective interpretations that require attention and discussion.
% \f{For example, }
% \zg{Too vague.}. The ability of humans to create plausible stories for even less likely scenarios results in diverse explanations and temporal spaces that differ subtly, expanding the task to more challenging settings.


% When humans are correct, the model succeeds 52\% of the time, suggesting a slight improvement in the models' likelihood of answering correctly 
% (see Appendix Figure ~\ref{fig:pp_true_exp_whoknows}).

 % both correct on average of 56\%.
%  when human correct, the chances for model to succeed 66\%. which might be easy to people is more likely to be easier to models.
%  when human is incorrect, the chances models will succeed is random (50\%).
%  totally the average human-model agreement is 64\%.

% The percentage of instances where the model is correct, but the human is not, is minimal (7\%). In such cases, it is uncommon for the model's explanation to be correct. Figure \mv{TODO: Fig} illustrates a rare example of this scenario. 

% When the model fails, only about 22\% of these failures are shared with humans, meaning both the model and the human answer incorrectly, implying on different types of errors in the common pattern thinking.

% When the model is correct, there are 89\% human success too, which 


% \mt{Suggestion instead of the previous paragraph: We calculate the number of samples where both humans and the model selected the same answer, regardless of correctness. We use the (\Separate, Triplet Setup) across all 350 examples. GPT-4O is excluded from this analysis due to its poor performance. On average, the agreement rate across models is 55\%, indicating that models and humans show some level of agreement, as two random baselines would have an expected agreement of 50\%. When separating the model results based on human correctness, we observe a slight improvement in the likelihood of a model answering correctly when humans are correct, and a significant drop (around 30\%) in accuracy when humans answer incorrectly, suggesting that when humans struggle, models tend to struggle as well.}

Figure \ref{fig:errors_heatmap} presents the percentage of error factors per model, highlighting several trends. Understanding temporal progression is a challenge for all models.  Claude predominantly relies on style considerations (30\%), whereas Gemini and GPT-4 often miss key details (32\%, 25\%). GPT-4 shows the highest rate of failed comparisons, indicating it engages in more logical and reasoning-based thinking, but fails primarily in plausibility comparison at the "last minute" decision point. diving more details, not in the heatmap), Claude struggles more with time duration compared to direction errors (\mv{4.4:1}), while Gemini and GPT-4 tend to make more direction errors (ratios of 1:1.45 and 1:2.83, respectively).

% \f{In addition, the models on average present 70\% logical explanation when they are correct. \mv{REPHRASE}}

% Appendix Figure~\ref{fig:false_pp_huamn_true_pp_model_exp_whoknows} illustrates a rare example of this scenario.



% Here, we qualitatively examine a subset of 120 explanations, 40 explanations from each VLM: Gemini 1.5, GPT-4, and Claude 3.5. Our focus is on explanations of incorrect hypothesis selections (\textit{Plausibility Prediction}) within the \separate input strategy (Triplet setup). Demonstrated by the following scenes (Figure \ref{fig:wet_floor}: premise, \textit{a man in a hospital bed with a broken leg}, and the two hypotheses, \textit{a wet floor with (less plausible) and without (plausible) a warning sign}, we find that the models' failures can be attributed to five main factors:

% (1) \textit{style \& consistency}. When irrelevant visual considerations lead to the decision (e.g., because the window in the background matches the one in the premise image); (2) \textit{time}. When the explanation relies on the wrong time direction or time duration. (e.g., assuming the hypothesis occurs after the premise, and concluding the sign was placed after an accident.); (3) \textit{ignored key details}.  overlooking key information (e.g., ignoring the cast on the man's leg, assuming he's resting rather than injured); (4) \textit{missing knowledge}. When the model recognizes key details, though without understanding their meaning correctly, misinterpreting (e.g., identifying the sign but not realizing it's a warning sign), and (5) \textit{failed comparison}. justifying the less plausible hypothesis with a logical explanation (e.g., the model selects the hypothesis with the warning sign, reasoning that the person might have been distracted and didn’t notice the sign, even though slipping could occur in either scenario).
% See examples in Appendix Figure \ref{fig:failure_explanations}.



% \begin{table}[ht]
% \centering
% \begin{minipage}{0.49\textwidth}
% \caption{Failure factors with examples, as illustrated by the following scene (Figure~ \ref{fig:wet_floor})—-with a premise of \textit{a man in a hospital bed with a broken leg} and two hypotheses: \textit{a wet floor with (less plausible) and without (plausible) a warning sign}.}
% \centering
% \scriptsize  % Use a smaller font size
% \begin{adjustbox}{width=0.95\textwidth}  % Adjust width for a smaller table
% \begin{NiceTabular}{p{0.35\textwidth} p{0.55\textwidth}} 
% \toprule
% \textbf{Failure Factor} & \textbf{Example} \\ 
% \midrule
% \textit{Style \& Consistency} & Selecting the image because the window in the background matches the one in the premise image. \\
% \midrule
% \textit{Time} & Assuming the hypothesis occurs after the premise and concluding the warning sign was placed after an accident. \\
% \midrule
% \textit{Ignored Key Details} & Ignoring the cast on the man's leg and assuming he’s resting rather than injured. \\
% \midrule
% \textit{Missing Knowledge} & Identifying the sign but not realizing it's a warning sign. \\
% \midrule
% \textit{Failed Comparison} & Selecting the hypothesis with the warning sign, reasoning the person was distracted and didn’t see it, even though slipping could occur in both cases. \\
% \bottomrule
% \end{NiceTabular}
% \end{adjustbox}
% \label{tab:failure_factors}
% \end{minipage}
% \hfill
% \begin{minipage}{0.49\textwidth}
% \centering
%   \includegraphics[width=0.95\textwidth]{figures/error_analysis_heatmap.pdf}
%   \captionof{figure}{Failure factors of model explanation for wrong plausibility predictions.}
%   \label{fig:errors_heatmap}
% \end{minipage}
% \end{table}


% Figure \ref{fig:errors_heatmap} presents the percentage of error factors per model, highlighting several trends. Understanding temporal progression is a challenge for all models.  Claude predominantly relies on style considerations (30\%), whereas Gemini and GPT-4 often miss key details (32\%, 25\%). GPT-4 shows the highest rate of failed comparisons, indicating it engages in more logical and reasoning-based thinking, but fails primarily in plausibility comparison at the "last minute" decision point. diving more details, not in the heatmap), Claude struggles more with time duration compared to direction errors (\mv{4.4:1}), while Gemini and GPT-4 tend to make more direction errors (ratios of 1:1.45 and 1:2.83, respectively).

% \f{In addition, the models on average present 70\% logical explanation when they are correct. \mv{REPHRASE}}




% \mt{
% Suggestion to replace the previous paragraph: 
% Here, we qualitatively examine a subset of 120 explanations for failure cases—40 explanations for each VLM: Gemini 1.5, GPT-4, and Claude 3.5. Our focus is on explanations of incorrect hypothesis selections (PP) within the \separate input strategy (Triplet setup). We find that the models' failures can be attributed to five main factors. 
% To demonstrate the different factors, let's examine a possible answer for the example in Figure \ref{fig:main_nl-eye}, where in the premise, there is a man in a hospital bed with a broken leg, and the two hypotheses are a wet floor with and without a warning sign.
% 1) relying on incorrect assumptions about \textit{time} direction or duration. For instance, assuming that the hypothesis occurs after the premise and, therefore, they would have learned from their mistakes and placed a warning sign.
% 2) relying on \textit{style or consistency} considerations, such as choosing the image with the warning sign because the window in the background is more similar to the window in the premise image.
% 3) \textit{missing knowledge} – recognizing the entities in the images without understanding their significance. For example, identifying the man with the broken leg, the wet floor, and the warning sign, but missing the fact that people are more likely to slip without warning sign.
% 4) \textit{failed comparison} – failure to choose the most probable scenario. For example, when the answer could be that the person could slip in both scenarios, the model incorrectly selects the one with the warning sign, reasoning that the person might have been distracted and therefore did not see the sign.
% 5) \textit{ignored key details} – for example, the model might overlook the fact that the man has a cast on his leg and instead suggest that the man is simply resting, thus concluding that there was probably a sign outside, since nobody was injured. See examples of the different factors in the Appendix Figure \ref{fig:failure_explanations}.
% }


% \mt{Correlations Are Easier Than Causation. -  Models score higher on cultural and social reasoning, compared to X. This might be due to the fast that this kind of reasoning mostly relies on specific niche knowledge (which models are highly proficient at). On the other hand...}

% \mt{
% Forward time reasoning is easier than backward - Reasoning over longer time frames and in a forward temporal direction tends to be easier for models compared to more complex causal relationships, like X, especially those that require reasoning backward (i.e. what leads to the premise scene) or over short-term intervals.
% }


% \begin{figure*} [!ht]
%   \centering
%   \includegraphics[width=0.8\textwidth]{figures/multiple_images_breakdowns.png}
%   \caption{Categories breakdowns of \separate input strategy: Reasoning Categories, Time Direction, Time Duration. Color notes Models-Baselines. Order of Reasoning Categories by Accuracy (low to high).}
%   \label{fig:category_all_in_one}
% \end{figure*}


% \begin{itemize}
%     \item multiple images average performance of API VLMs (40.5\%) similar to \combined (43\%).
%     \item GPT-4o is significantly better at \combined (54\% difference) while Claude 3.5 and Gemini better at multiple images with 8\% and 21\% differences, correspondingly.
%     \item Open-source VLMs, Claude 3, and GPT 4o (multiple) scores below random or around it.
%     \item dumb pixel baseline scores higher than most of the models.
%     \item Humans outperform models aggressively
%     \item There are order preferences for each model with significant accuracy differences (see table \ref{tab:consistency_models})
% \end{itemize}



% \mv{Human IAA: fleiss kappa: 0.32 (fair), 3 total agree: 67.6\%}



==> reasoning.tex <==



==> related_work_backup.tex <==
\section{Related Work}
\label{sec:related_work}

\mv{relevent work to add: MMToM-QA: https://arxiv.org/abs/2401.08743}

\yb{Another related work (I think for the related work section): fu2024commonsense https://arxiv.org/html/2406.07546v1}
% VLM
Significant advancements in the fields of Natural Language Processing (NLP) and Computer Vision (CV) have enabled the processing of textual and visual inputs separately across diverse tasks \cite{qin2024large, guo2022attention, voulodimos2018deep}.
Large Language Models (LLMs) development along with the improvement of visual encoders such as CLIP \cite{clip_radford2021learning, openclip_cherti2022reproducible} and SigLip \cite{zhai2023sigmoid}, has led to the development of modality conversion models such as Text-To-Image \citep{rombach2021highresolution_sd, ramesh2022hierarchical_dalle2}, Image-To-Text models and Visual-Question-Answering (VQA) \cite{li2023blip, dai2023instructblip}. In recent years, Visual Language Models (VLMs) have emerged \cite{google2024gemini, claude2024, achiam2023gpt, liu2024llavanext, liu2024visual, bai2023qwen}, enabling the integration of both modalities as inputs or outputs, thus standing at the forefront of these advancements.

% \paragraph{Commonsense Reasoning in Visual Language Models.}
Many studies explore reasonable inference processes in multimodal setups. In these setups, A VLM receives a textual prompt grounded in visual input, which can be a single image or multiple images. Most commonsense research on single images focuses on visual-text alignment, asking straightforward questions about an object in the image \C{}. Other studies focus on prompts that integrate a specific cue related to the examined phenomenon (e.g., "What is weird in the image?") or about a localized visual cue related to the expected reasoning (e.g., "There is smoke.").

When the grounding consists of multiple images, the complexity level is higher due to the required combination of basic computer vision capabilities such as recognition and tracking, along with higher-level reasoning abilities like temporal sense and understanding of physical and social dynamics. Multiple images as visual grounding have been mainly explored in video generation \C{} and next action prediction \C{SEEDBench}. While this line of work often focuses on short-term sequences, we also include long-term sequences in both directions. 
Additionally, this research is mostly based on natural images extracted from open sources such as YouTube or online image datasets \C{VCOPA}. In our setup, we have the ability to synthesize any scene without dependence on existing sources. This enables us to control the difficulty level and parameters to examine reasoning capabilities in a more controlled environment while maintaining a photorealistic style. 

Other recent work related to spatial reasoning involves questions accompanied by multiple diagrams or schemes \C{NTSEBench} as complementary help to the question or as multiple possible answers \C{ScienceQA}. While this research is focused on mathematical-scientific-data analytics setups, we propose more daily-life reasoning that can be utilized in day-to-day applications. 

\bench\ is a dataset that is entirely end-to-end human-made,  ensuring highly consistent and high-quality images compared to those extracted from various sources. The synthetic generation of the images in the benchmark also offers a flexible and enabling framework for any scene to be included and expended.\bench\ uniquely allows for the examination of reasoning capabilities across multiple domains and provides a scalable evaluation framework for setups involving a larger number of images.







% input format: single image VS multiple images
% type of question content:  phenomenon, cue, visual-text alignment
% images / annotation: natural-human versus synthetic-model
% task format - answers format: 2 hypothesis, open-answer, 
% prompting (format question: CoT, 
% temporal refrence

%Another approach...
%Inspired by that idea
%compared to <models>
%<X were the first to...
% in contrast our work


\yb{\textbf{Commonsense Reasoning in VLMs.} Commonsense reasoning in Visual Language Models (VLMs) has been extensively studied, with benchmarks like Visual Commonsense Reasoning (VCR) \cite{zellers2019recognition} challenging models to infer underlying situations in images. Single-image tasks such as Sherlock \cite{hessel2022abduction}, WHOOPS! \cite{bitton2023breaking}, and Visual Riddles \cite{bitton2024visualriddles} push models to interpret complex cues and unusual scenarios, often generated using text-to-image models. Fu et al. \cite{fu2024commonsense} highlight significant limitations in current VLMs' abilities to perform tasks requiring deep understanding of the physical world. Our work builds upon these studies by introducing a benchmark that tests abductive reasoning across diverse reasoning categories—including physical, social, and cultural domains—and temporal dimensions like forward and backward reasoning. Unlike prior efforts focusing on single-image scenarios, our dataset requires models to reason across multiple images, capturing temporal sequences and causal relationships essential for comprehensive commonsense reasoning.}

\yb{Furthermore, by leveraging text-to-image generation models like DALL·E  and Midjourney, we synthesize high-quality, photorealistic images tailored to specific reasoning challenges. This synthetic approach allows us to create controlled and consistent visual data, enabling the systematic exploration of reasoning capabilities that are difficult to assess using natural images alone.}
